QD-BEV : Quantization-aware View-guided Distillation for Multi-view 3D Object Detection

Multi-view 3D detection based on BEV (bird-eye-view) has recently achieved significant improvements. However, the huge memory consumption of state-of-the-art models makes it hard to deploy them on vehicles, and the non-trivial latency will affect the real-time perception of streaming applications. Despite the wide application of quantization to lighten models, we show in our paper that directly applying quantization in BEV tasks will 1) make the training unstable, and 2) lead to intolerable performance degradation. To solve these issues, our method QD-BEV enables a novel view-guided distillation (VGD) objective, which can stabilize the quantization-aware training (QAT) while enhancing the model performance by leveraging both image features and BEV features. Our experiments show that QD-BEV achieves similar or even better accuracy than previous methods with significant efficiency gains. On the nuScenes datasets, the 4-bit weight and 6-bit activation quantized QD-BEV-Tiny model achieves 37.2% NDS with only 15.8 MB model size, outperforming BevFormer-Tiny by 1.8% with an 8x model compression. On the Small and Base variants, QD-BEV models also perform superbly and achieve 47.9% NDS (28.2 MB) and 50.9% NDS (32.9 MB), respectively.

==> latex/sec/sec1_noref.tex <==
\section{Introduction}
\label{sec:intro}
 % Considering the high latency and low efficiency of BEVFormer, we come up with a new architecture with quantization and distillation which can make low-bits model obtain the same performance of full-precision version. 
   % We observe the correlation between BEV feature and image feature, so 
   % we construct the view-guided distillation loss and use it to lead the direction of gradient descent, promoting the effect of QAT. We analyzes the contribution of different view of camera respectively when calculating BEV Feature, and we generate the view-depended BEV mask and apply it to distillation loss.
\renewcommand{\dblfloatpagefraction}{.9}
\begin{figure*}[htp]
\centering
      \includegraphics[width=0.95\linewidth]{latex/figure/figure1.png}
   \caption{\t   extbf{Illustration of QD-BEV.} In our pipeline, multi-camera images are input into the floating-point teacher network and the quantized student network in order to compute the KL divergence in an element-wise manner. The KL divergence is used as distillation loss in the image feature and the BEV feature, respectively. Then we conduct view-guided distillation using the BEV mask obtained from the external parameters of the camera.
   The lower flow chart shows the computation process of the view-guided distillation loss.
   }
   \label{fig:intro}
\end{figure*}

% Limitation of existing works:

% 1.BEV tasks have considerable resource consumption.

% 2.high-performance networks cannot be really deployed.

% 3.Direct low-bit quantization of the network will greatly reduce the accuracy.

% Problem statement : Improving Efficiency and Reduce Consumption in Multi-view Camera based 3D Detection.

% 1.Make Low-bit Quantization feasible on BEV tasks.

% 2.Design a unique Distillation framework for the BEV tasks.

% 3.Improve the performance of the Lower-bit model by distillation.

% Proposed method : Efficient BEV Architecture which is A BEV perception Model with high Efficiency and low Energy Consumption.
%  Obtaining high-precision and low-bit quantization model through QAT and KD. The student model obtained by KD can greatly reduce the loss of accuracy while maintaining superior performance.

% Contributions:

% Proposed a Efficient BEV architecture based on Multi-view vision camera .

% First to implement low-bit quantization on BEV tasks .

% Unique View-Guided Distillation Architecture on BEV tasks .



% 基于BEV（鸟瞰图）的3D目标检测是自动驾驶领域和深度学习领域的一个重要方向，基于传感器可分为激光雷达和相机模态的方法。尤其是基于相机的方法，由于它具有部署成本低、更贴近人眼的特征，以及便于获取驾驶环境中的视觉元素信息等优势，是当下研究的热点。然而即便相较于激光雷达的方法，基于相机的方法已经节省了很多成本，但是大型的BEV网络需要的计算成本依然相当庞大，这使得网络很难被部署到载具上。因此，探究BEV网络的轻量化工作变得尤为重要。

% 在传统的图像分类和目标检测任务中，为了得到更加轻盈的网络，进行的网络的轻量化工作主要有，剪枝，量化，和知识蒸馏，有一些轻量化方法在传统的任务中取得了不错的效果。然而多相机3D检测任务比传统的图像分类和目标检测任务的复杂度和困难度要大非常多，一般会通过更深层的卷积神经网络作为backbone提取多个view的图像信息，再配合复杂的transformer结构来编码和解码BEV领域的特征。在简单任务上比较有效的模型轻量化方法在迁移到复杂任务上可能并不能获得比较好的效果。





Given its potential in enabling autopilot, camera-only 3D detection based on BEV (bird-eye-view)
%3D object detection based on BEV (bird-eyes-view) 
has became an important research direction for autonomous driving. 
Based on input sensors, previous work can be divided into LiDAR-based methods \cite{lang2019pointpillars,zhou2018voxelnet} and camera-only methods \cite{li2022bevformer,wang2022detr3d,huang2021bevdet,huang2022bevdet4d,liu2022petr,liu2022petrv2}.
Compared to the LiDAR-based methods, camera-only methods have the merits of lower deployment cost, closer to human eyes, and easier access to visual information in the driving environment.
However, even if using the camera-only methods, the computational costs of running state-of-the-art BEV models are still formidable, making it difficult to deploy the model onto vehicles. For example, 
%BEVFormer-Base \cite{li2022bevformer} requires 28 GB of memory for training and it takes 14 days to finish a 24-epoch training process on one NVIDIA A100 GPU. Moreover, 
BEVFormer-Base has a 540 ms inference latency (corresponds to 1.85 fps) on one NVIDIA V100 GPU, which is infeasible for real-time applications that generally require 30 fps.
% 用BEVFormer-base网络来举例，他需要每张GPU上28G的显存，在单张tesla-A100的GPU上对它进行训练完成24个epoch需要14天的时间。
Therefore, it is particularly crucial to explore and devise lightweight models for camera-only 3D object detection based on BEV.

Model compression methods, such as quantization~\cite{jacob2018quantization, gholami2021survey}, pruning~\cite{han2015deep, dong2017learning, yu2022hessian}, and knowledge distillation~\cite{hinton2015distilling, yin2020dreaming}, are widely used in traditional computer vision tasks to obtain more compact models.
Since major obstacles against deploying BEV networks include long on-device inference latency and large model size, we pioneer the usage of quantization to obtain smaller BEV models.
Quantization can reduce the bitwidth used to represent weights and activations in deep neural networks, which can greatly save the model size and computational costs while improving the speed of model reasoning.
However, directly applying quantization would lead to significant performance degradation. 
Compared to image classification and 2D object detection tasks where the standard compression methods shine, multi-camera 3D detection tasks are much more complicated and difficult due to the existence of multiple views and information from multiple dimensions (for example, the temporal information and spatial information used in BEVFormer~\cite{li2022bevformer}). Consequently, the structure of BEV networks tends to become more complex, with a deeper convolutional neural network backbone to extract image information from multiple views, and transformers to encode and decode the features of the BEV domain. The presence of different neural architectures and operations greatly challenges the standard quantization methods, decreasing their stability and accuracy, and even making the whole training process diverge.

% 现有的BEV相关工作中，有一些工作聚焦在efficient上，但是目前并没有已发表的工作聚焦在BEV任务的quantization上。量化可以极大节省模型大小和显存消耗，8bit可以减小4倍，4bit可以减小8倍，并极大提升模型推理速度，对模型实际的部署来说是非常必要的。



% 在BEV领域的蒸馏上，我们注意到了一些工作是通过知识蒸馏的方式把激光雷达的信息教给基于相机的网络，但是对激光雷达数据的额外要求也与纯相机的理念相悖。目前也并没有纯相机的知识蒸馏工作。

% 在这篇工作中，我们提出了一种针对BEV任务设计的量化感知知识蒸馏方法，通过img feature和 bev feature 的映射关系，构建一套将BEV模型量化到低比特位宽并能保持精度甚至超过浮点精度的方法。如图所示，我们将fp模型作为teacher模型，将我们预训练得到的低比特量化模型作为student模型，分别在img feature和bev feature 上去计算kl 散度，再通过相机外参将RGB特征和BEV特征两部分有机的结合起来实现我们特有的View Guided Distillation方式，将量化后模型的精度提升至浮点模型水平。

% 在我们的工作中先尝试采用传统的量化方式对模型直接进行ptq和qat，在比特数较低时这样会带来极大的精度损失。因此为BEV模型设计行之有效的低比特量化方式是充满挑战和吸引力的。值得注意的是，在我们的量化和蒸馏过程中，始终是在相同维度的模型上做的。我们并没有为了更好的实验结果采用额外的训练数据或更大的模型去tricky地提升模型精度，我们只使用了原始的训练数据和原本的浮点模型。


To solve the aforementioned problems, in this work, we first conduct systematic experiments and analyses on quantizing BEV networks. Then we devise a quantization-aware view-guided distillation method (referred to as QD-BEV) that can decently solve the stability issue of standard QAT while improving the final performance of compact BEV models.
Our proposed view-guided distillation (VGD) can better leverage information from both the image and the BEV domains, which can significantly outperform previous distillation methods which cannot jointly handle the different types of losses in BEV networks.
As shown in Figure~\ref{fig:intro}, we construct our QD-BEV pipeline leveraging the mapping relationship between the image feature and the BEV feature.
Specifically, we first take the FP (floating-point) model as the teacher model and the low-bit quantized model as the student model, then we calculate the KL divergence on the image feature and the BEV feature, respectively. 

% \zhen{@Yifan we need a better explanation on this Finally... sentence after you update the figure.}
Finally, we realize our unique View-Guided Distillation (VGD) by organically combining the image feature and the BEV feature through the camera's external parameters. Note that in our QD-BEV pipeline, neither additional training data nor larger powerful teacher networks are used to tune the accuracy, but QD-BEV models are still able to outperform previous baselines while having a significantly smaller model size and computational requirements.
% In our work, we first try to use the traditional quantization method to post training quantization and quantization aware training the model directly, which will bring a great loss of accuracy when the number of bits is low. 
% Therefore, it is challenging and attractive to design an effective low-bit quantization method for the BEV model. 
% It is worth noting that in our quantization and distillation process, it is always done on the model of the same dimension. 
Our contributions are as follows:
\begin{itemize}
    \item We pioneer the use of quantization to obtain QD-BEV, a family of efficient models for camera-only 3D object detection based on BEV.
    \item We conduct systematic experiments on quantizing BEV models, unveiling major issues hampering standard quantization-aware training methods on BEV. 
    \item We propose view-guided distillation (VGD), which jointly leverages both image domain and BEV domain information. VGD boosts QAT performance by solving the stability issue of standard QAT. 
    \item The resulted QD-BEV outperforms previous baselines while being significantly smaller. The W4A6 quantized QD-BEV-Tiny has 37.2\% NDS with an only 15.8 MB model size, which outperforms the 8$\times$ larger BevFormer-Tiny model by 1.8\%.
\end{itemize}




==> latex/sec/sec3_noref.tex <==
\section{Method}
% 在这部分我们先概括的介绍一下我们的工作，再详细介绍我们的View guided Distillation 和 progressive quantization aware training 方法。

In this section, we first give an overview of our work, then introduce our view-guided distillation and progressive quantization-aware training methods in detail.

\subsection{Overview of QD-BEV pipeline}
\label{subsec:overview of qd-bev}

% 在这个部分我们先回顾一下channel-wise Distillation [1]的方法, 这篇论文的框架展示在图一中。我们有一个全精度的教师网络和一个量化过的学生模型，其中学生模型是通过我们针对BEV任务设计的渐进式量化感知训练得到的。输入的多相机图像分别进入教师和学生模型，在网络的Backbone和neck部分之后我们提取到提取多相机的图片特征，在网络的transformer部分之后提取到BEV特征。取得这几部分特征之后，我们在教师模型和学生模型的两部分特征分别去做蒸馏，再通过相机外参将两部分蒸馏融合得到我们独有的View-guided Distillation机制。

This work aims to improve the efficiency of state-of-the-art BEV architecture. Start with the widely applied BEVFormer architecture~\cite{li2022bevformer}, we propose a progressive quantization aware training procedure to quantize the cumbersome BEVFormer models into the efficient QD-BEV models in a stage-by stage fashion. Specifically, we start the model training with a high quantization precision, while gradually quantize more model stages into low precision during the QAT process. 
After achieving the fully quantized QD-BEV model, we further boost its performance through a novel view-guided distillation process, which is highlighted in~\cref{fig:intro}. 
We use a full-precision teacher model to facilitate the learning of our quantized QD-BEV student model.
The input multi-camera image is entered into the teacher and student model respectively, and then the  $Image Backbone$ and $Image Neck$ parts of the network are used to extract the multi-camera image feature.  After the transformer part of the network, the BEV features are extracted, and the two parts of the teacher model and student model are distilled respectively. After obtaining these features, we distilled the two parts of the teacher model and the student model respectively, and then fused the two parts of distillation through the external parameters of the camera to get our unique View-guided Distillation mechanism. Through our overall process, we can finally get a low-bit quantization model with accuracy comparable to full accuracy.
We provide detailed formulation of the view-guided distillation process in section View-guided distillation.
% ~\cref{subsec:vgd}.





\subsection{Progressive quantization-aware training}
\label{sec:PQAT}

In symmetric linear quantization, the quantizer maps weights and activations into integers with a scale factor $S$. Uniformly quantizing to k bit can be expressed as:
\begin{equation}
\begin{split}
%\begin{aligned}
\textit{S} =\frac{2|r_{\max}|}{2^{k}-1},\ 
% Z_{0} &=\operatorname{round}\left(2^{k-1}-1-\frac{r_{\max }}{S}\right) \\
\textit{q} =\textit{round}\left(\frac{r}{S}\right),
%\end{aligned}
\end{split}
\end{equation}
\normalsize
where $r$ is the floating-point number being quantized, $|r_{\max}|$ is the largest absolute value in $r$, and $q$ is the quantized integer.
% In baseline methods, we use symmetric quantization, which means $Z_0$ equals 0 and the first bit of $Z$ serves as a sign bit, with the rest k-1 bits used to represent the integer.
% There are usually two types of quantization methods: post-training quantization (PTQ) and quantization-aware training (QAT). 
In this work, we conduct systematic experiments to analyze the performance of quantization on BEV networks. For PTQ, we apply the above quantization directly to the pre-trained models during the inference stage. For QAT, we utilize the straight-through estimator (STE)~\cite{bengio2013estimating} to define the forward and backward pass for the above quantization operations and train the model to better adapt to quantization. Both methods are useful and can be applied to different circumstances for deployment.


% Compared with the floating-point precision model, the quantized model can greatly reduce the hardware resources consumed by the model, and the quantization of the model is indispensable in the Industrial deployment. 
% However, the existing multi-camera-based BEV models consume a lot of resources and can not be deployed at all, so it is necessary to quantify the models with low bits.
% 现有的量化方法中
% （学长介绍一下PTQ和QAT和我们采用的HAWQ方法以及我们为什么采用hawq&maybe说明我们输入第一层w8a8以及对multiheadattn不做量化or这个说明我们放在之后的实验细节？）

% \zhen{@Yifan move these to experiments if needed. We first try to do ptq to the model, the accuracy loss of direct post-training quantization is very large, in 6bit weight and 6bit activation, the gap between the quantized model and the full accuracy has been quite large (more than 15 percentage points).
% changing the quantization parameters such as the clipping interval of the model can slightly improve this phenomenon, but it still can not fundamentally recover the accuracy loss caused by quantization.
% We still need quantization aware training to change the weight of the model for different quantized bit widths.}
% % 接下来我们讨论一下我们Progressive Quantization aware training的工作细节。

% % 直接对模型做QAT在较高比特也许是可行的，比如8比特权重8比特激活和6比特权重16比特激活.它们由于量化引入的量化噪声比较少，在ptq就可以获得还不错的精度，直接采用QAT会较为容易的找到收敛的方向。但是当视角来到更低比特的量化，如6比特权重6比特激活和4比特权重6比特激活，引入的量化噪声远大于高比特的模型，直接ptq的精度损失非常大，qat的能力是有限的，没有办法找到收敛的正确方向，直接引入训练好的浮点精度模型的权重作为初始化亦或是从头开始训练都会在几个epoch的训练之后发生梯度爆炸，训练崩坏。
% % Next, let's discuss the details of our Progressive Quantization aware training work.

% \zhen{if needed, move to experiments. It may be feasible to Quantization aware training the model directly at higher bits, such as 8-bit activation with 8-bit weight and 16-bit activation with 6-bit weight. Because of the less quantization noise introduced by quantization, they can achieve good accuracy in post-training quantization, and it is easier to find the direction of convergence by using Quantization aware training directly. However, when the angle of view comes to the quantization of lower bits, such as 6-bit activation and 4-bit activation, the quantization noise introduced is much larger than that of the high-bit model, the accuracy loss of direct post-training quantization is very large, and the ability of Quantization aware training is limited, so there is no way to find the right direction of convergence.}

As discussed in above, due to the complexity of multi-camera 3D object detection tasks and of the BEV networks, directly quantizing the model to ultra-low bit-width may incur sub-optimal and unstable training, even gradient explosion. To solve this problem, we introduce progressive QAT which reduces the quantization influence with a two-fold process. First, we propose to reach the target bit-width in a progressive way. Instead of directly quantizing the network to the final scheme of 4-bit weights and 6-bit activations (W4A6), we first quantize it to W32A6. The quantization perturbation from W32A32 to W32A6 is significantly smaller than the perturbation from W32A32 to W4A6, which can intrinsically address the issue of performance drop and gradient explosion. Furthermore, the W32A6 models has significantly higher learning capacity than the W4A6 models, which helps the progressive roadmap from W32A32 to W32A6 to W4A6 to learn smoothly and obtain better-optimized models.
% can get better pretrain at each step, reduce the quantization noise at each step, and reduce the pressure on Quantization aware training.
% 为了解决上述问题，我们可以采用两种方向的Progressive Quantization aware training。
% 第一种是在位宽层面逐渐从高比特向低比特量化，比如先训练一个w6a8的模型，用这个模型的权重作为w6a6模型的pretrain，再训练出w6a6的模型，以此类推。我们将fp模型作为pretrain来做低比特模型的量化训练可以看作是粗粒度的位宽层面的Progressive Quantization aware training，即从32bit直接到低比特。更细粒度的操作可以在每一步获得更好的pretrain，让每一步的量化噪声更小，减轻QAT的压力。

% The first is to gradually quantify from high bit to low bit at the bit width level, for example, first train a 6-bit weight and 8-bit activation model, use the weight of this model as the pretrain of the 6-bit weight and 6-bit activation model, then use Quantization aware training to train the 6-bit weight and 6-bit activation model, and so on. 
% We use floating point model as pretrain to do quantitative training of low-bit model, which can be regarded as coarse-grained bit width level Progressive Quantization aware training, that is, from 32-bit directly to low bit. 

% 第二种是在结构层面从前往后逐步量化网络的各个部分。我们把BEVFormer的网络分成四个部分，backbone，neck，encoder，decoder。Progressive Quantization的顺序是根据输入图片在神经网络中传播的顺序决定的。我们先对backbone做量化，网络中别的部分保持全精度，进行混合精度的量化训练。精度收敛之后我们再对neck做量化，重复上面的步骤，以此类推。最终我们得到了整网都量化过的高精度低比特网络。
Secondly, when converting the model from W32A6 to W4A6, we propose a stage-wise progressive quantization to gradually reducing the weight precision stage-by-stage.
% gradually quantify all parts of the network from front to back at the structural level. 
Specifically, we follow the design of BEVFormer~\cite{li2022bevformer} to consider four stages: backbone, neck, encoder, and decoder. 
% The order of Progressive Quantization is determined by the order in which the input pictures are propagated in the neural network. 
We first quantize the backbone to W4A6 while keeping the other stages W32A6, and perform QAT on this mixed-precision model. 
% and carry on the mix-precision quantization aware  training. 
After the QAT converges, we move on to the next stage of QAT where the neck precision is also reduced.
Iterative, we can obtain a fully quantized low-bit network at the end. This fully-quantized model serves as the starting point for our QD-BEV model, after which we further boost the performance using the novel view-guided distillation method.
% 在我们得到了整网都量化过的预训练模型之后，就可以采用上一节提到的View Guided Distillation方法提升量化后模型的精度，最终获得高精度的低比特量化模型。

% After we get the pre-training model which has been quantized by the whole network,









\subsection{View-guided distillation}
\label{subsec:vgd}
% BEV网络的结构最鲜明的特点是，它有提取RGB的Feature过程，也有生成BEVFeature的过程。因此我们在对BEV网络进行蒸馏的时候同时要考虑到两个层面的信息，将他们有机的结合起来而不是简单的加权相加。设计专门针对BEV网络结构的独特蒸馏方法。
The most distinct characteristics of the BEV networks are the joint process of extracting both image features and BEV features.
Therefore, when distilling the BEV networks, it is crucial to jointly consider the two levels of information and combine them organically, rather than simply adding or stacking them together. 
In the following sections, we present details of our proposed view-guided distillation, the computation of which requires the image feature distillation, the BEV feature distillation, and joining the information.

\subsubsection{Image feature distillation}
\label{subsec:img_feature}

% 我们首先对齐教师和学生网络，在img feature上进行第一步的蒸馏。我们分别提取fp的教师网络和低比特量化的学生网络的的img neck的输出作为我们要蒸馏的图像特征。这是一个有5个维度的tensor，分别是batch size, number of cameras, channel, height, width. 然后我们可以将学生和老师的feature转成概率分布， 就可以通过kl散度来衡量它们之间的差异。我们先对feature做softmax，如公式所示。
Given a pair of aligned teacher and student model,
We first compute element-wise distillation loss on image features.
We extract the image neck output as the image features to be distilled. 
To improve the smoothness of the distillation loss, we follow previous attempts~\cite{shu2021channel} to use a KL divergence-based distillation loss.
Specifically, we consider the flattened image features of the student and the teacher model as logits, which we convert into probability distribution via a softmax function with temperature $\phi_{\tau}$, as defined in~\cref{eq:softmax_ImgFeature_t}.

\begin{equation}
	{\phi_{\tau}(x_i)} = \frac{e^{x_i/\tau}}{\sum_j e^{x_{j}/\tau}}.
	\label{eq:softmax_ImgFeature_t}
\end{equation}

% 然后我们对每个相机的输出分别计算它们的kl散度。如公式所示。
Then we calculate the KL divergence of each camera's output separately to achieve the image feature distillation loss, as in~\cref{eq:Loss_img}.
\begin{equation}
    \begin{split}
    {\mathcal{L}_{img}} = \frac{\tau ^2}{{ B}\cdot { W}\cdot { H}\cdot { C}} \times \mathcal{D}_{KL} \left( \phi_{\tau}(F^{T}_{img}),\phi_{\tau}(F^{S}_{img}) \right),
	\label{eq:Loss_img}
    \end{split}
\end{equation}
where B means batchsize, W means imgFeature width, H means imgFeature height, C means imgFeature Channel, and 
$F^{T}_{img}$ and $F^{S}_{img}$ denotes the imgFeature of teacher model and student model respectively.

\subsubsection{BEV feature distillation}
\label{subsec:bev_feature}


% 我们在BEV feature上进行第二步的蒸馏。我们分别提取fp的教师网络和低比特量化的学生网络的的生成的BEV feature。这是一个有3个维度的tensor，分别是$ BEV_H * BEV_W$，batch size, channel.和对img feature的操作一样，先将学生和老师的feature转成概率分布， 然后通过kl散度来衡量它们之间的差异。

We carried out the second step of distillation on BEV feature. 
As with image features, the BEV features of student and teacher are first converted into a probability distribution.
% 然后我们对BEVFeature上的每个点去计算KL散度
Then we calculate the KL divergence for each point on the BEV seature, as shown in~\cref{eq:Loss_BEV}.
\begin{equation}
    \begin{split}
    {\mathcal{L}_{bev}} = \frac{\tau ^2}{{ B}\cdot { C}} \times {\rm \mathcal{D}_{KL}} \left( \phi_{\tau}(F^{T}_{bev}),\phi_{\tau}(F^{S}_{bev}) \right),
	\label{eq:Loss_BEV}
    \end{split}
\end{equation}
where B means batchsize, C means BEVFeature Channel, and 
$F^{T}_{bev}$ and $F^{S}_{bev}$ denotes the BEV Feature of teacher model and student model respectively. We get a loss with shape of $[ H_{bev} \times W_{bev}, 1]$. 



\subsubsection{View-guided distillation objective}
\label{subsec:compute_vgd}
% 在前两小节中，我们获得了Img feature 上每个相机的loss ，也获得了BEV feature上每个点对应的loss。

% 在nuscenes数据集上，相机外参是已知的，因此我们可以通过相机外参得到每个相机对应到BEVfeature上的分布范围，即$BEV mask$ ，和BEVFormer中的定义相同。

% $BEV mask$ 是一个有4个维度的tensor，分别是 $number of camera，batch size， BEV_H * BEV_W，3D Height $ , 每一个元素是 True 或 False。我们把最后一维压缩，就得到了2d平面上的BEV_mask.

%  通过$BEV mask$ 就可以将 针对每个相机算出来的${Loss_{img}}$ 拓展到针对BEV feature上的每个点对应的loss，即{Masked\underline{~}Loss_{img}}
In the first two sections, we obtained the loss of each camera on the Img feature and the corresponding loss of each point on the BEV feature. 
On the nuScenes data set, the camera external parameters are known, so we can get the distribution range of each camera corresponding to the BEV feature. Then we generate the mask of views which can be applied to the image feature, that is, $M_{bev}$, which is the same as defined in BEVFormer~\cite{li2022bevformer}.  
$M_{bev}$ is a tensor with four dimensions: number of cameras, batch size, BEV Size$(H_{bev} \times W_{bev})$, and 3D Height, with binary values in each element. 
Flattening the last 2 dimensions gives the $M_{bev}$ on the 2d plane. 
With $M_{bev}$, the ${\mathcal{L}_{img}}$ calculated for each camera can be extended to the corresponding loss for each point on the BEV feature, that is, 
${\widehat{\mathcal{L}}_{img}}$.

\begin{equation}
\begin{split}
{\widehat{\mathcal{L}}_{img}} = {\mathcal{L}_{img}} \odot M_{bev}
\label{eq:masked img loss}
\end{split}
\end{equation}

$ M_{bev} $ is calculated from the camera external parameters, and it is a tensor with the shape of $[6, H_{bev} \times W_{bev}]$, which indicates the range of BEVfeature affected by each camera. $\odot$ in~\cref{eq:masked img loss} denotes the hadamard product.

% 最终再通过这个 {Masked\underline{~}Loss_{img}} 去引导${Loss_ {img}$  得到了最终的由每个View的img distill信息去引导的BEV distill 的View Guided Distillation

Finally, we use ${\widehat{\mathcal{L}}_{img}}$ to get the final BEV distill objective, View Guided Distillation, which is guided by the image distill information of each view in~\cref{eq:View Guided Loss}

\begin{equation}
\begin{split}
\mathcal{L}_{vgd} ={\sum_{i=1}^{N\cdot H\cdot W}} {\widehat{\mathcal{L}}_{img}} \odot {\mathcal{L}_{bev}}
\label{eq:View Guided Loss}
\end{split}
\end{equation}

The overall process of view-guided distillation is shown in Algorithm~\ref{algorithm1}.

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
% \begin{algorithm}
% %\small
%         \caption{View-Guided Distillation}
%         \label{algorithm1}
%         \begin{algorithmic}[1]
%             \Require 
%             $BEV\underline{~}mask$ caculated by camera external params\\
%             ImgFeature of Teacher and Student : $F^S_{img} $, $F^T_{img}$\\
%             BEVFeature of Teacher and Student : $F^S_{bev} $, $F^T_{bev}$
%             \Ensure View-Guided Distillation Loss : $L_{vgd}$
%             \State Initialize losses: $L_{i}, L_{B}, Masked\underline{~}L_{i} $ and $L_{vgd}$
%             \State Set temperature parameter for ImgFeature and BEVFeature: $\tau_{i} , \tau_{b} $
%             \For {$i$ in iterations}
%                     \State Update $L_{i}$ by calculate the KL divergence of  $F^S_{img} $ and $F^T_{img}$ with $\tau_{i}$ \ref{eq:Loss_img}
%                     \State Update $L_{B}$ by calculate the KL divergence of $F^S_{bev} $ and $F^T_{bev}$ with $\tau_{b}$ \ref{eq:Loss_BEV}
%                     \State Update $Masked\underline{~}L_{i}$ by introduce location information into $L_{i}$ by $BEV\underline{~}mask$ \ref{eq:masked img loss}
%                     \State Update $L_{vgd}$ by multiply $Masked\_L_{i}$ and  $L_{B}$ \ref{eq:View Guided Loss}
%             \EndFor
%         \State {\bfseries end for }
%         \State \textup{return} $L_{i}, L_{B}, Masked\underline{~}L_{i} $
%         \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
% %\small
%         \caption{View-Guided Distillation}
%         \label{algorithm1}
%         \begin{algorithmic}[1]
%             \Require 
%             $BEV\underline{~}mask$ caculated by camera external params\\
%             ImgFeature of Teacher and Student : $F^S_{img} $, $F^T_{img}$\\
%             BEVFeature of Teacher and Student : $F^S_{bev} $, $F^T_{bev}$
%             \Ensure View-Guided Distillation Loss : $L_{vgd}$
%             \State Initialize losses: $L_{i}, L_{B}, Masked\underline{~}L_{i} $ and $L_{vgd}$
%             \State Set temperature parameter for ImgFeature and BEVFeature: $\tau_{i} , \tau_{b} $
%             \For {$i$ in iterations}
%                     \State $L_{i}$ = KLD ( $F^S_{img}$ , $F^T_{img}$ ; $\tau_{i}$ ) \ref{eq:Loss_img}
%                     \State $L_{b}$ = KLD ( $F^S_{bev}$ , $F^T_{bev}$ ; $\tau_{b}$ )
%                     \State Update $Masked\underline{~}L_{i}$ by introduce location information into $L_{i}$ by $BEV\underline{~}mask$ \ref{eq:masked img loss}
%                     \State Update $L_{vgd}$ by multiply $Masked\_L_{i}$ and  $L_{B}$ \ref{eq:View Guided Loss}
%             \EndFor
%         \State {\bfseries end for }
%         \State \textup{return} $L_{i}, L_{B}, Masked\underline{~}L_{i} $
%         \end{algorithmic}
% \end{algorithm}




\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[t]
        \caption{\text{Progressive Quantization-Aware VGD}}
        \begin{algorithmic}[1]
            \Require Training data; 
            \\ Pre-trained FP weights for teacher model $T_{fp}$; 
            \\ student model $S$; 
            \\ Numbers of epochs for each phase $N_1$, ... , $N_4$; $P_2$;
            \\ Quantization bit for weight and activation $B_w; B_a$
            \Ensure Trained low-bit student weight $S_q$ % with bit width $Bit_w;Bit_a$ 
% stage 1
        \State \textbf{Phase 1: Progressive Quantization-Aware Training} 
        \State Init $S_{0}$ with $T_{fp}$; Divide model into a 4 dim $Parts$ : 
                $\lbrace Backbone, Neck, Encoder, Decoder \rbrace$;
        \For{$i, module$ in $Parts$}{}
            % \State Set quantize bit in $module$ to $B_w$, $B_a$
            \State $module$ = quantize ( $module$; $B_w$, $B_a$ )
            \State Init $S_{i}$ with $S_{i-1}$
            \For{Epoch = $N_{i-1}$ ,..., $N_i$}{ }
                \State Update $S_{q_i}$ by minimizing QAT loss %using backpropagation
            \EndFor
        \EndFor
        \State \textbf{Phase 2: View-Guided Distillation} 
        \State Init ${S}$ with $S_{4}$  %; 
        \For{ Epoch = 1, ... , $P_2$} 
            \State Update $S$ by minimizing QAT loss and $\mathcal{L}_{vgd}$ in~\cref{eq:View Guided Loss}
        \EndFor
        \end{algorithmic}
\label{algorithm1}
\end{algorithm}









==> latex/sec/sec4_noref.tex <==
\section{Experiments}
\label{sec:Exp}

%-------------------------------------------------------------------------
In this section, we first elaborate on the experimental settings, then we evaluate both PTQ and QAT methods on the BEV networks. 
% performance of QD-BEV under different size models and different bit width task targets, and
Based on the analysis of these results, we propose QD-BEV to overcome shortcomings in PTQ and QAT, and we dedicatedly compare our results with previous works under different settings and constraints.
\subsection{Experimental settings}
\subsubsection{Dataset}

% 我们在大规模公共数据集nuScenes上进行3d 检测任务的实验，nuScenes是由Motional(前身为nuTonomy)的团队开发的用于自动驾驶的公共大型数据集，它包括在波士顿和新加坡收集的1000个人工选择的20秒长的驾驶场景。其中750个场景为训练集，100个为验证集，150个为测试集。数据集中的相机图像采集自6个已知内外参的相机。

We conduct experiments on 3D detection tasks using a large-scale public dataset nuScenes \cite{caesar2020nuscenes}, a large public dataset for autopilot developed by the team of Motional (formerly nuTonomy), which includes 1000 manually selected 20-second driving scenarios collected in Boston and Singapore. 
Among them, 750 scenarios are training sets, 100 are verification sets, and 150 are test sets. 
The images in the dataset are collected from 6 cameras with known internal and external parameters.


\begin{table*}[!t]
\tiny
\vspace{-3pt}
% \small
\renewcommand\arraystretch{1}
    \centering
    \caption{Results with  PTQ separately applied on each part in BEVFormer.}
    \label{tab: part Result}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cccc|cc|cc|cc} 
\toprule
% \hline 
 \multicolumn{4}{c|}{Quantized Module}  & \multicolumn{2}{c|}{BEVFormer-Tiny} & \multicolumn{2}{c|}{BEVFormer-Small} & \multicolumn{2}{c}{BEVFormer-Base} \\
\midrule
Backbone& Neck& Encoder& Decoder & mAP↑ & NDS↑ & mAP↑ & NDS↑ & mAP↑ & NDS↑ \\
\midrule % xxxx
\fontsize{4pt}{24pt}\XSolid & \fontsize{4pt}{24pt}\XSolid & \fontsize{4pt}{24pt}\XSolid & \fontsize{4pt}{24pt}\XSolid & 0.252 & 0.354 & 0.370 & 0.479 & 0.416 & 0.517\\

\midrule
% oxxx
\fontsize{5pt}{24pt}\CheckmarkBold & \fontsize{4pt}{24pt}\XSolid & \fontsize{4pt}{24pt}\XSolid & \fontsize{4pt}{24pt}\XSolid & 0.212 & 0.310 & 0.288 & 0.417 & 0.309 & 0.440\\

% xoxx
\fontsize{4pt}{24pt}\XSolid & \fontsize{5pt}{24pt}\CheckmarkBold & \fontsize{4pt}{24pt}\XSolid & \fontsize{4pt}{24pt}\XSolid & \bf{0.252} & \bf{0.353} & \bf{0.370} & \bf{0.478} & \bf{0.416} & 0.516  \\

% xxox
\fontsize{4pt}{24pt}\XSolid & \fontsize{4pt}{24pt}\XSolid & \fontsize{5pt}{24pt}\CheckmarkBold & \fontsize{4pt}{24pt}\XSolid & 0.181 & 0.295 & 0.298 & 0.421 & 0.160 & 0.303\\

% xxxo
\fontsize{4pt}{24pt}\XSolid & \fontsize{4pt}{24pt}\XSolid & \fontsize{4pt}{24pt}\XSolid & \fontsize{5pt}{24pt}\CheckmarkBold & 0.251 & \bf{0.353} & 0.369 & 0.477 & \bf{0.416} & \bf{0.517}\\
\midrule
% oooo
\fontsize{5pt}{24pt}\CheckmarkBold & \fontsize{5pt}{24pt}\CheckmarkBold & \fontsize{5pt}{24pt}\CheckmarkBold & \fontsize{5pt}{24pt}\CheckmarkBold & 0.145 & 0.246 & 0.228 & 0.369 & 0.075 & 0.224\\
% \hline 
\bottomrule
\end{tabular}
}
\end{table*}

\subsubsection{Evaluation metrics}

% 对模型量化压缩的工作来说，模型大小和BOPS是重要的衡量指标。我们的工作主要实在nuScenes 3d 检测数据集上进行实验和评估的，因此主要的衡量指标有mean Average Precision (mAP)，和nuScenes数据集特有的评估指标nuScenes detection score (NDS)，这是一个包含了很多方面信息的综合性评价指标。其余的衡量指标有mean Average Translation Error (mATE), mean Average Scale Error (mASE), mean Average Orientation Error (mAOE), mean Average Velocity Error (mAVE) 以及mean Average Attribute Error (mAAE)。
% 
The main measurement indicators on the nuScenes 3D test dataset are the mean Average Precision (mAP), and the unique evaluation index nuScenes detection score (NDS). NDS is a comprehensive evaluation index containing many aspects of information. 
The other indicators are mean Average Translation Error (mATE), mean Average Scale Error (mASE), mean Average Orientation Error (mAOE), mean Average Velocity Error (mAVE) and mean Average Attribute Error (mAAE).

% For the work of model quantification and compression, model size and BOPS are important indicators.
To evaluate the efficiency of the BEV networks, we use model size and BOPS as the metrics. 
Model size is the memory required to store a specific network, which is determined by the total amount of parameters in the model as well as the quantization bitwidth to store those parameters.
BOPS measures the total Bit Operations(BOPS) for calculating a layer~\cite{van2020bayesian}. It is a common metric for evaluating the computation of quantized neural networks. For a model with $L$ layers, defining $b_{w_i}$ and $b_{a_i}$ to be the bit precision used for weights and activations of the $i$-th layer, then we have:
\begin{equation}
\begin{split}
\textit{BOPS} = \sum\nolimits_{i=1}^L b_{w_i}b_{a_i} \textit{MAC}_i
\end{split}
\end{equation} 
where MAC$_i$ is the total Multiply-Accumulate operations for computing the $i$-th layer.


\subsubsection{Baselines}

% 我们主要与 BEVFormer 的三种不同输入图像分辨率和backbone的模型，BEVFormer-tiny, BEVFormer-small,BEVFormer-base的fp模型进行对比。同时也与相同输入分辨率和backbone的 SRCN3D，PETR， BEVDet4D作为参考。

We mainly compare with floating-point baseline models proposed by BEVFormer~\cite{li2022bevformer} with different input image resolutions (specifically, BEVFormer-Tiny, BEVFormer-Small and BEVFormer-Base).
% 我们也将DFQ的量化方法应用在BEVFormer上做INT8训练后量化作为我们量化方面的baseline。
For quantization baselines, we apply a previous PTQ method DFQ~\cite{nagel2019data} as well as a QAT method HAWQv3~\cite{yao2021hawq} to BEVFormer models.
% At the same time, it is also used as a reference with PETR and BEVDet of the same input resolution and backbone.

% \vspace{-11pt}

\subsubsection{Implementation details}

% 对浮点模型，根据BEVFormer的开源仓库，我们采用了两种不同的backbone：ResNet50，ResNet101-DCN，对应三种不同大小的模型：BEVFormer-tiny, BEVFormer-small, BEVFormer-base.采用BEVFormer开源的全精度权重checkpoint. 

For floating-point models, we use the open-sourced repository of BEVFormer, and we use two different backbones: ResNet50 and ResNet101-DCN. 
We use symmetrical linear quantization in a channel-wise manner for weights, and layer-wise for activations. 
Since there is little related work in our settings for reference, we make our training adopt the same scheme as the original training strategy of BEVFormer, which is to train 24 epoch in each step, and to use Optimizer of AdamW, a starting lr as 2e-4, a linear warmup of 500 iters, and cosine annealing.
Due to limited computational resources, we tend to finish the stages ahead of time in the progressive QAT. As such, even higher accuracy can potentially be gained with more dedicated training processes. 
% Considering the time of the experiment, we will finish this stage ahead of time and start the next stage in some steps, which may lead to not converging to the optimal solution. 
% Therefore, if we reproduce our work and strictly follow the given time to converge each step to the optimal solution, may get better results than we do.
% 4bit weight and 6bit activation are used to quantify the target bit width set, and other quantization settings are also used as reference experiments.
% corresponding to three different sizes of models: BEVFormer-tiny, BEVFormer-small, BEVFormer-base. 
% We use BEVFormer open source full-precision weight checkpoint.

% 在量化方式上我们采用的是HAWQ-v3的量化框架.量化方式为perchannel的对称量化。量化目标位宽集中采用了4bit权重和6bit激活，也采用了别的量化设置作为参考实验。

% In the way of quantization, we use the quantization framework of HAWQ-v3. 

% 由于很少有相关的工作作为参考，我们试探性的让每一步的训练采用与BEVFormer原本的训练策略相同的训练方案，每一步训练24个epoch，并且采用AdamW的Optimizer，起始lr为2e-4，采用500个iters的线性warmup和余弦退火。综合对实验时间的考量，我们在某些步骤会提前结束这个阶段并开始下一个阶段，这可能会导致没有收敛到最优解。因此如果复现我们的工作并严格按照给定的时间去让每一步都收敛到最优解，可能会得到比我们更好的结果。



\begin{table}[ht]
\caption{PTQ results with different quantization bitwidth.}
\vspace{-5pt}
\label{table:ptq results}
% \setlength{\tabcolsep}{7.5pt}  
\centering
\resizebox{0.86\linewidth}{!}{
\begin{tabular}{c | c c c c c}
\toprule
% \hline
W-bit/A-bit            & Model   & NDS↑  & NDS Drop  &  mAP↑    \\ 
\hline
% 32/32
\multirow{3}{*}{32/32}  & Tiny   & 0.354 &     -     & 0.252 \\ 
                        & Small  & 0.479 &     -     &  0.370  \\
                        & Base   & 0.517 &     -     &  0.416  \\
\midrule
% 8/8
\multirow{3}{*}{8/8}    & Tiny   & 0.351 &   0.8\%    &  0.248  \\ 
                        & Small  & 0.477 &   0.4\%    &  0.366  \\
                        & Base   & 0.487 &   5.8\%    &  0.384  \\
% \multirow{3}{*}{8/8}    &  tiny  & 0.351(-0.003) &  0.248(-0.004)  \\ 
%                         & small  & 0.477(-0.002) &  0.366(-0.004)  \\
%                         & base   & 0.487(-0.030) &  0.384(-0.032)  \\
\midrule
% 6/6
\multirow{3}{*}{6/6}    & Tiny   & 0.312 &   11.9\%    &  0.203  \\ 
                        & Small  & 0.430 &   10.2\%    &  0.306  \\
                        & Base   & 0.402 &   22.2\%    &  0.262  \\
% \multirow{3}{*}{6/6} & tiny   & 0.312(-0.042) &  0.203(-0.048)  \\ 
%                         & small  & 0.430(-0.049) &  0.306(-0.064)  \\
%                         & base   & 0.402(-0.115) &  0.262(-0.154)  \\
\midrule
% 4/6
\multirow{3}{*}{4/6}    & Tiny   & 0.246 &   30.5\%    &  0.146  \\ 
                        & Small  & 0.369 &   23.0\%    &  0.228  \\
                        & Base   & 0.226 &   56.3\%    &  0.076  \\
% \multirow{3}{*}{4/6} & tiny   & 0.246(-0.108) &  0.146(-0.106)  \\ 
%                         & small  & 0.369(-0.110) &  0.228(-0.142)  \\
%                         & base   & 0.226(-0.291) &  0.076(-0.340)  \\
\midrule
% 4/4
\multirow{3}{*}{4/4}    & Tiny   & 0.034 &   90.4\%    &  0.001  \\ 
                        & Small  & 0.034 &   92.9\%    &  0.001  \\
                        & Base   & 0.023 &   95.6\%    &  0.000  \\
% \multirow{3}{*}{4/4}    & tiny   & 0.034(-0.320) &  0.001(-0.251)  \\ 
%                         & small  & 0.034(-0.445) &  0.001(-0.365)  \\
%                         & base   & 0.023(-0.494) &  0.000(-0.416)  \\
% \hline
\bottomrule
\end{tabular}}
\vspace{-7pt}
\end{table}






\subsection{QD-BEV Results and Analysis}
\input{latex/table/table_main.tex}





\subsubsection{PTQ results}

% 我们先对模型做了不同bit的ptq。
% 从表一可以观察到对模型直接做ptq会带来非常严重的精度损失，尤其是对激活做量化时，6it就会有0.15以上的NDS和mAP掉点。
% 我们为了更精细的观察每一个部分的量化给模型带来的精度损失，对每个部分分别单独做量化，去观察原浮点模型在不同bit下的表现。
% 从表二可以发现......网络的backbone 和 encoder 部分比较敏感， 而neck 和 decoder 由于包含的卷积层和线性层较少，对它们做量化后，对网络的精度只带来比较轻微的扰动。

We first analyze the sensitivity of different modules to quantization in Table~\ref{tab: part Result}. It can be seen that the backbone and the encoder parts of the network are more sensitive, while quantization of the neck and the decoder parts only brings a slight disturbance to the accuracy. We want to note that, based on the sensitivity analysis, it is possible to apply mixed-precision quantization to better preserve the sensitive modules, which can be beneficial to the trade-off between model size and the final accuracy.
% because they contain less convolution layer and linear layer.

We then analyze the influence of different quantization bitwidth on post-training quantization. 
In Table \ref{table:ptq results}, directly applying PTQ with less than 8-bit precision will lead to a significant accuracy drop, especially when quantized to W4A4 the results become pure noise with around 0 mAP. As can be observed from Table~\ref{table:ptq results}, performing QAT is necessary in order to preserve the accuracy while achieving ultra-low bit quantization. 
% In order to observe the precision loss of the model caused by the quantization of each part, we quantize each part to 4 bit weight and 6 bit activation separately to observe the performance of the original floating point model under different bit. 



% \vspace{-10pt}
\subsubsection{Progressive QAT results}

\begin{figure*}[htp]
\centering
      \includegraphics[width=0.95\linewidth]{latex/figure/figure_sec4/progressive2.pdf}
   \caption{\textbf{Progressive QAT.} 
   \textbf{} We observe that the precision loss may become intolerable when we quantize the model in one step. Thus, we propose progressive quantization-aware training which divides the quantization of the whole model into many phases. Progressive QAT can significantly improve the stability of QAT as well as the accuracy it achieves. The pink line in the figure represents the baseline NDS.
   }
   \label{fig:progressive}
\end{figure*}

% 由之前的ptq实验观察到BEV模型的敏感度，我们选定4/6bit 权重，6bit激活作为我们的量化目标。

% 我们先对模型的整网进行QAT实验。 由于w6a6已经与fp的模型引入了非常大的量化误差，所以直接对fp模型进行整网的量化会给QAT带来很大的难度，训练会有很大的不确定性和不可控性。 训练会在一些时候进入一些奇异值点导致梯度爆炸，精度快速下降。我们尝试进行梯度裁剪的操作，可以延缓梯度爆炸现象的发生但并不能从根本上解决问题，模型依然无法达到我们需要的精度。

% （配一个梯度爆炸的图？）

% From the previous PTQ experiments to observe the sensitivity of the BEV model, 
Since PTQ cannot achieve ultra-low precision, we aim to apply QAT for 4-bit quantization. 
% First, we do QAT experiments on the whole network of the model. 
% Because w6a6 has introduced a very large quantization error with the fp model, directly quantifying the whole network of the fp model will bring great difficulty to the QAT, and the training will have great uncertainty and uncontrollability. 
From all our experiments, standard QAT methods which directly quantize the whole network to the target bitwidth will lead to unstable QAT processes, resulting in a gradient explosion and a rapid decline in accuracy.
% We try to carry out the operation of gradient clipping, which can delay the occurrence of gradient explosion, but it can not fundamentally solve the problem, and the model still can not achieve the accuracy we need. 
% \textcolor{blue}{It may be feasible to Quantization aware training the model directly at higher bits, such as 8-bit activation with 8-bit weight and 16-bit activation with 6-bit weight. Because of the less quantization noise introduced by quantization, they can achieve good accuracy in post-training quantization, and it is easier to find the direction of convergence by using Quantization aware training directly. However, when the angle of view comes to the quantization of lower bits, such as 6-bit activation and 4-bit activation, the quantization noise introduced is much larger than that of the high-bit model, the accuracy loss of direct post-training quantization is very large, and the ability of Quantization aware training is limited, so there is no way to find the right direction of convergence.}


% 由于上述原因，我们根据模型的结构采用progressive quantization aware training进行模型训练。我们先在tiny模型上进行w4a6实验，如图所示。
% 可以观察到由于我们分割了量化带来的误差到每一步上，减轻了每一步的压力，从而使得QAT可以找到正确的收敛方向。

% Because of the above reasons, 
Consequently, we propose to use progressive QAT to constrain the quantization perturbation along the training process. 
As an example, we plot the training curve of our progressive QAT in Figure \ref{fig:progressive}, where we conduct W4A6 quantization on the BEVFormer-Tiny. We separate the progressive QAT into 4 stages and iteratively quantize a new module in each stage. As can be seen, there is an NDS drop at the beginning of each stage, corresponding to the quantization perturbation introduced by the quantized new module. We should note that progressive QAT is able to effectively recover the NDS drop, and the final results obtained purely with progressive QAT are discussed in the ablation study.
% It can be observed that because we divide the error caused by quantization to each step, the pressure of each step is reduced, so that QAT can find the correct convergence direction.

\begin{figure}[t]
  \centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=4.4cm]{latex/figure/figure_sec4/map-curve.pdf}
    \caption{mAP curve.}
    \label{fig:tiny_map}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=4.4cm]{latex/figure/figure_sec4/nds-curve.pdf}
    \caption{NDS curve.}
    \label{fig:tiny_nds}
  \end{subfigure}
    \centering
  \caption{Training curve of view-guided distillation versus QAT on W4A6 quantization of BEVFormer-Tiny.}
  \label{fig:vgd curve}
\end{figure}

\subsubsection{View-guided distillation results}
% 在progressive quantization aware training的基础上，我们为了获得更好的精度，就可以用QAT训练出来的w4a6模型作为student model，以fp模型为teacher model进行 view Guided Distillation. tiny 模型进行4bit weight 6bit activation 的VGD的效果如图所示。

% 可以看到VGD为模型带来非常稳定平滑的loss下降曲线，并且模型的NDS和mAP精度提升也非常显著。达到了惊人的0.3708的NDS和0.2541的mAP。超过QAT的结果0.3478的NDS和0.2339的mAP 两个点以上，甚至达到了比原有fp模型更好的精度，如表所示。

Although progressive QAT is significantly superior to standard QAT, it still suffers from fluctuation during training, as shown in Figure~\ref{fig:vgd curve}. In order to obtain better accuracy and stability, we apply view-guided distillation with the floating-point model as the teacher and the quantized model as the student. The effect of VGD on W4A6 quantization of BEVFormer-Tiny is shown in Figure~\ref{fig:progressive}.
It can be seen from both figures that VGD can bring a very stable and significant improvement to the model. Benefiting from knowledge in both the image domain and the BEV domain, QD-BEV networks are able to fully recover the quantization degradation, and even outperform the floating-point baselines. As shown in Table~\ref{tab: sota all}, the NDS and mAP of the model outperform previous floating-point baselines as well as quantized networks. Note that since there are no existing results for compact BEV networks, we implement standard quantization methods DFQ~\cite{nagel2019data} and HAWQv3~\cite{yao2021hawq} on BEVFormer as a comparison. 
We apply W8A8 quantization for DFQ (DFQ with lower bitwidth has intolerable accuracy degradation) and W4A6 for all QD-BEV models.
% The result of exceeding QAT is more than 0.3478 NDS and 0.2339 mAP, and even achieves better accuracy than the original fp model, as shown in the table.
As a comparison, QD-BEV can achieve 0.493 NDS with only 33 MB model size, which is similar to the size of BEVFormer-T-DFQ (0.340 NDS) and much smaller than BEVFormer-Tiny (126.8 MB, 0.354 NDS).
In Figure~\ref{fig:visual1}, we show the visualization results of the QD-BEV-Base model on the nuScenes val dataset, and compare them with the results of BEVFormer-Tiny and the ground truth. 
% QD-BEV-Base has achieved a much better prediction than BEVFormer-Tiny under 1/4 model size, 
As can be seen, more objects are detected by QD-BEV-Base, and the 3D bboxes predictions are more accurate than BEVFormer-Tiny. More visualizations are provided in the supplementary material.





% \begin{figure*}[t]
%   \centering
%   \begin{subfigure}{0.49\linewidth}
%     \includegraphics[width=8.8cm]{latex/figure/figure_sec4/map-curve.pdf}
%     \caption{mAP curve.}
%     \label{fig:tiny_map}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.49\linewidth}
%     \includegraphics[width=8.8cm]{latex/figure/figure_sec4/nds-curve.pdf}
%     \caption{NDS curve.}
%     \label{fig:tiny_nds}
%   \end{subfigure}
%     \centering
%   \caption{Training curve of view-guided distillation versus QAT on W4A6 quantization of BEVFormer-Tiny.}
%   \label{fig:vgd curve}
% \end{figure*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{latex/figure/figure_sec4/Visual1.png}
    \caption{Visualization of QD-BEV results and the comparison with results obtained by BEVFormer.}
    \label{fig:visual1}
\end{figure}





% small和base模型的VGD结果等待补充。

% \begin{figure}[t]
% \includegraphics[width=8.2cm]{latex/figure/tiny_vd_mAP.png}
% \centering
% \caption{\textbf{Network architecture of }. }
% \label{fig:3}
% %\vspace{-10pt}
% \end{figure}








==> latex/table/table_rebuttal.tex <==

% \begin{table*}[!t]
% \scriptsize
% \renewcommand\arraystretch{1.5}
%     \centering
%     \caption{\bf{QD-BEV results compared to previous methods or baselines.}}
%     \label{tab: sota all}
% \resizebox{0.92\linewidth}{!}
% {
% \begingroup
%     \setlength{\tabcolsep}{2pt}
% \begin{tabular}{c|c|cc|cc|ccccc} 
% \toprule
% Input Size & Model & Model Size(MB) & BOPS(Tera) & NDS↑  & mAP↑  & mATE↓  & mASE↓  & mAOE↓  & mAVE↓  & mAAE↓   \\ 
% \midrule
% % \multirow{2}{*}{384$\times$1056} & BEVDet-R50\cite{huang2021bevdet} & 203.3 & 94.11 & 0.381 & 0.304 & 0.719  & 0.272  & 0.555  & 0.903  & 0.257   \\
% %                                  & PETR-R50\cite{liu2022petr} & -  & - & 0.381 & 0.313 & 0.768  & 0.278  & 0.564  & 0.923  & 0.225   \\ 
% % \hline
% % \multirow{4}{*}{450$\times$800}  & BEVFormer-T\cite{li2022bevformer} & 126.8  & 62.33 & 0.354 & 0.253 & 0.899  & 0.294  & 0.655  & 0.657  & 0.216   \\
% %                                  & BEVFormer-T-DFQ\cite{nagel2019data}  & 31.7 & 3.90 & 0.340 & 0.236 & 0.949  & 0.296  & 0.651  & 0.671  & 0.217   \\
% %                                  & BEVFormer-T-HAWQv3\cite{yao2021hawq} & 15.9 & 1.46 & 0.348 & 0.234 & 0.949 & 0.304 & 0.568 & 0.661 & 0.209   \\
% %                                  \rowcolor{orange!40}\cellcolor{orange!0}& QD-BEV-T (Ours)  & 15.9 & 1.46 & 0.372 & 0.255 & 0.882  & 0.321  & 0.543  & 0.599  & 0.214   \\ 
% % \midrule
% % \multirow{2}{*}{512$\times$1408} & PETR-R101\cite{liu2022petr} & - & - & 0.421 & 0.357 & 0.710 & 0.270 & 0.490 & 0.885 & 0.224 \\
% %                                  & PETR-Tiny & -  & - & 0.431 & 0.361 & 0.732 & 0.273 & 0.497 & 0.808 & 0.185  \\ 
% % \hline
% \multirow{4}{*}{720$\times$1280} & BEVFormer-S-DFQ\cite{nagel2019data} & 56.4 & 14.76 & 0.467 & 0.356 & 0.751  & 0.283  & 0.405  & 0.451  & 0.222 \\
%                                  & BEVFormer-S-HAWQv3\cite{yao2021hawq} & 28.2 & 5.53 &  0.467 & 0.356 & 0.751 & 0.287 & 0.419 & 0.449 & 0.208 \\
%                                  & BEVFormer-S-PACT\cite{choi2018pact} & 28.2 & 5.53 &  0.461 & 0.351 & 0.750 & 0.275 & 0.422 & 0.507 & 0.196 \\
%                                  \rowcolor{orange!40}\cellcolor{orange!0}& QD-BEV-S (Ours) & 28.2 & 5.53 & 0.479 & 0.374 & 0.716 & 0.290 & 0.389 & 0.474 & 0.210 \\ 
% % \midrule
% % \multirow{4}{*}{900$\times$1600} & DETR3D\cite{wang2022detr3d} & 195.7 & 520.60 & 0.425 & 0.346 & 0.773  & 0.268  & 0.383  & 0.842  & 0.216 \\
% %                                  & PETR-r101\cite{liu2022petr} & - & - & 0.455 & 0.391 & 0.647  & 0.251  & 0.433  & 0.933  & 0.143 \\
% %                                  & FCOS3D\cite{wang2021fcos3d} & 200.3 & 1028.20 & 0.415 & 0.343 & 0.725  & 0.263  & 0.422  & 1.292  & 0.153 \\
% %                                  & SRCN3D-r101\cite{shi2022srcn3d} & - & - & 0.428 & 0.337 & 0.779  & 0.287  & 0.367  & 0.781  & 0.188 \\ 
% \hline
% \multirow{4}{*}{900$\times$1600} & BEVFormer-B-DFQ\cite{nagel2019data} & 65.7 & 41.71 & 0.486 & 0.384 & 0.771  & 0.274  & 0.378 & 0.427 & 0.206 \\
%                                  & BEVFormer-B-HAWQv3\cite{yao2021hawq} & 32.9 & 15.64 &  0.485 & 0.376 & 0.727 & 0.288 & 0.381 & 0.434 & 0.202 \\
%                                  & BEVFormer-B-PACT\cite{choi2018pact} & 32.9 & 15.64 &  0.480 & 0.374 & 0.735 & 0.291 & 0.392 & 0.458 & 0.201 \\
%                                  \rowcolor{orange!40}\cellcolor{orange!0} & QD-BEV-B (Ours) & 32.9 & 15.64 & 0.493 & 0.393 & 0.707 & 0.286 & 0.425 & 0.416 & 0.203 \\
% \bottomrule
% \end{tabular}
% \endgroup 
% }
% \end{table*}


\begin{table}[!t]
\scriptsize
\renewcommand\arraystretch{1.5}
    \centering
    \caption{\bf{QD-BEV results compared to QAT baseline.}}
    \vspace{-1em}
    \label{tab: rebuttal table}
\resizebox{0.8\linewidth}{!}
{
\begingroup
    \setlength{\tabcolsep}{2pt}
\begin{tabular}{c|c|cc|cc} 
\toprule
Input Size & Model & W & A & NDS  & mAP\\ 
\midrule
% \multirow{2}{*}{384$\times$1056} & BEVDet-R50\cite{huang2021bevdet} & 203.3 & 94.11 & 0.381 & 0.304 & 0.719  & 0.272  & 0.555  & 0.903  & 0.257   \\
%                                  & PETR-R50\cite{liu2022petr} & -  & - & 0.381 & 0.313 & 0.768  & 0.278  & 0.564  & 0.923  & 0.225   \\ 
% \hline
% \multirow{4}{*}{450$\times$800}  & BEVFormer-T\cite{li2022bevformer} & 126.8  & 62.33 & 0.354 & 0.253 & 0.899  & 0.294  & 0.655  & 0.657  & 0.216   \\
%                                  & BEVFormer-T-DFQ\cite{nagel2019data}  & 31.7 & 3.90 & 0.340 & 0.236 & 0.949  & 0.296  & 0.651  & 0.671  & 0.217   \\
%                                  & BEVFormer-T-HAWQv3\cite{yao2021hawq} & 15.9 & 1.46 & 0.348 & 0.234 & 0.949 & 0.304 & 0.568 & 0.661 & 0.209   \\
%                                  \rowcolor{orange!40}\cellcolor{orange!0}& QD-BEV-T (Ours)  & 15.9 & 1.46 & 0.372 & 0.255 & 0.882  & 0.321  & 0.543  & 0.599  & 0.214   \\ 
% \midrule
% \multirow{2}{*}{512$\times$1408} & PETR-R101\cite{liu2022petr} & - & - & 0.421 & 0.357 & 0.710 & 0.270 & 0.490 & 0.885 & 0.224 \\
%                                  & PETR-Tiny & -  & - & 0.431 & 0.361 & 0.732 & 0.273 & 0.497 & 0.808 & 0.185  \\ 
% \hline
\multirow{4}{*}{720$\times$1280} & BEVFormer-S-DFQ\cite{nagel2019data} & 8 & 8 & 0.467 & 0.356  \\
                                 & BEVFormer-S-HAWQv3 & 4 & 6 &  0.467 & 0.356 \\
                                 & BEVFormer-S-PACT\cite{choi2018pact} & 4 & 6 &  0.461 & 0.351 \\
                                 \rowcolor{orange!40}\cellcolor{orange!0}& QD-BEV-S (Ours) & 4 & 6 & \textbf{0.479} & \textbf{0.374} \\ 
% \midrule
% \multirow{4}{*}{900$\times$1600} & DETR3D\cite{wang2022detr3d} & 195.7 & 520.60 & 0.425 & 0.346 & 0.773  & 0.268  & 0.383  & 0.842  & 0.216 \\
%                                  & PETR-r101\cite{liu2022petr} & - & - & 0.455 & 0.391 & 0.647  & 0.251  & 0.433  & 0.933  & 0.143 \\
%                                  & FCOS3D\cite{wang2021fcos3d} & 200.3 & 1028.20 & 0.415 & 0.343 & 0.725  & 0.263  & 0.422  & 1.292  & 0.153 \\
%                                  & SRCN3D-r101\cite{shi2022srcn3d} & - & - & 0.428 & 0.337 & 0.779  & 0.287  & 0.367  & 0.781  & 0.188 \\ 
\hline
\multirow{4}{*}{900$\times$1600} & BEVFormer-B-DFQ\cite{nagel2019data} & 8 & 8 & 0.486 & 0.384 \\
                                 & BEVFormer-B-HAWQv3 & 4 & 6 &  0.485 & 0.376 \\
                                 & BEVFormer-B-PACT\cite{choi2018pact} & 4 & 6 &  0.480 & 0.374 \\
                                 \rowcolor{orange!40}\cellcolor{orange!0} & QD-BEV-B (Ours) & 4 & 6 & \textbf{0.493} & \textbf{0.393} \\
\bottomrule
\end{tabular}
\endgroup 
}
\vspace{-2em}
\end{table}



% \begin{table*}[!t]
% \scriptsize
% \renewcommand\arraystretch{1.5}
%     \centering
%     \caption{\bf{QD-BEV results compared to previous methods or baselines.}}
%     \label{tab: sota all}
% \resizebox{0.92\linewidth}{!}
% {
% \begingroup
%     \setlength{\tabcolsep}{2pt}
% \begin{tabular}{c|c|cc|cc|ccccc} 
% \toprule
% Input Size & Model & W & A & NDS↑  & mAP↑  & mATE↓  & mASE↓  & mAOE↓  & mAVE↓  & mAAE↓   \\ 
% \midrule
% % \multirow{2}{*}{384$\times$1056} & BEVDet-R50\cite{huang2021bevdet} & 203.3 & 94.11 & 0.381 & 0.304 & 0.719  & 0.272  & 0.555  & 0.903  & 0.257   \\
% %                                  & PETR-R50\cite{liu2022petr} & -  & - & 0.381 & 0.313 & 0.768  & 0.278  & 0.564  & 0.923  & 0.225   \\ 
% % \hline
% % \multirow{4}{*}{450$\times$800}  & BEVFormer-T\cite{li2022bevformer} & 126.8  & 62.33 & 0.354 & 0.253 & 0.899  & 0.294  & 0.655  & 0.657  & 0.216   \\
% %                                  & BEVFormer-T-DFQ\cite{nagel2019data}  & 31.7 & 3.90 & 0.340 & 0.236 & 0.949  & 0.296  & 0.651  & 0.671  & 0.217   \\
% %                                  & BEVFormer-T-HAWQv3\cite{yao2021hawq} & 15.9 & 1.46 & 0.348 & 0.234 & 0.949 & 0.304 & 0.568 & 0.661 & 0.209   \\
% %                                  \rowcolor{orange!40}\cellcolor{orange!0}& QD-BEV-T (Ours)  & 15.9 & 1.46 & 0.372 & 0.255 & 0.882  & 0.321  & 0.543  & 0.599  & 0.214   \\ 
% % \midrule
% % \multirow{2}{*}{512$\times$1408} & PETR-R101\cite{liu2022petr} & - & - & 0.421 & 0.357 & 0.710 & 0.270 & 0.490 & 0.885 & 0.224 \\
% %                                  & PETR-Tiny & -  & - & 0.431 & 0.361 & 0.732 & 0.273 & 0.497 & 0.808 & 0.185  \\ 
% % \hline
% \multirow{4}{*}{720$\times$1280} & BEVFormer-S-DFQ\cite{nagel2019data} & 8 & 8 & 0.467 & 0.356 & 0.751  & 0.283  & 0.405  & 0.451  & 0.222 \\
%                                  & BEVFormer-S-HAWQv3\cite{yao2021hawq} & 4 & 6 &  0.467 & 0.356 & 0.751 & 0.287 & 0.419 & 0.449 & 0.208 \\
%                                  & BEVFormer-S-PACT\cite{choi2018pact} & 4 & 6 &  0.461 & 0.351 & 0.750 & 0.275 & 0.422 & 0.507 & 0.196 \\
%                                  \rowcolor{orange!40}\cellcolor{orange!0}& QD-BEV-S (Ours) & 4 & 6 & 0.479 & 0.374 & 0.716 & 0.290 & 0.389 & 0.474 & 0.210 \\ 
% % \midrule
% % \multirow{4}{*}{900$\times$1600} & DETR3D\cite{wang2022detr3d} & 195.7 & 520.60 & 0.425 & 0.346 & 0.773  & 0.268  & 0.383  & 0.842  & 0.216 \\
% %                                  & PETR-r101\cite{liu2022petr} & - & - & 0.455 & 0.391 & 0.647  & 0.251  & 0.433  & 0.933  & 0.143 \\
% %                                  & FCOS3D\cite{wang2021fcos3d} & 200.3 & 1028.20 & 0.415 & 0.343 & 0.725  & 0.263  & 0.422  & 1.292  & 0.153 \\
% %                                  & SRCN3D-r101\cite{shi2022srcn3d} & - & - & 0.428 & 0.337 & 0.779  & 0.287  & 0.367  & 0.781  & 0.188 \\ 
% \hline
% \multirow{4}{*}{900$\times$1600} & BEVFormer-B-DFQ\cite{nagel2019data} & 8 & 8 & 0.486 & 0.384 & 0.771  & 0.274  & 0.378 & 0.427 & 0.206 \\
%                                  & BEVFormer-B-HAWQv3\cite{yao2021hawq} & 4 & 6 &  0.485 & 0.376 & 0.727 & 0.288 & 0.381 & 0.434 & 0.202 \\
%                                  & BEVFormer-B-PACT\cite{choi2018pact} & 4 & 6 &  0.480 & 0.374 & 0.735 & 0.291 & 0.392 & 0.458 & 0.201 \\
%                                  \rowcolor{orange!40}\cellcolor{orange!0} & QD-BEV-B (Ours) & 4 & 6 & 0.493 & 0.393 & 0.707 & 0.286 & 0.425 & 0.416 & 0.203 \\
% \bottomrule
% \end{tabular}
% \endgroup 
% }
% \end{table*}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
%\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
%\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

